PVN3D: A Deep Point-wise 3D Keypoints Voting Network for 6DoF Pose Estimation

In this work, we present a novel data-driven method for robust 6DoF object pose estimation from a single RGBD image. Unlike previous methods that directly regressing pose parameters, we tackle this challenging task with a keypoint-based approach. Specifically, we propose a deep Hough voting network to detect 3D keypoints of objects and then estimate the 6D pose parameters within a least-squares fitting manner. Our method is a natural extension of 2D-keypoint approaches that successfully work on RGB based 6DoF estimation. It allows us to fully utilize the geometric constraint of rigid objects with the extra depth information and is easy for a network to learn and optimize. Extensive experiments were conducted to demonstrate the effectiveness of 3D-keypoint detection in the 6D pose estimation task. Experimental results also show our method outperforms the state-of-the-art methods by large margins on several benchmarks. Code and video are available at https://github.com/ethnhe/PVN3D.git.

==> intro_old.tex <==
\section{INTRODUCTION}

In this paper, we study the problem of 6DoF pose estimation, i.e. recognize the 3D location and orientation of an object in a canonical frame.  It is an important component in many real-world applications, such as robotic grasping and manipulation \cite{collet2011moped,tremblay2018deep,zhu2014single}, autonomous driving \cite{geiger2012we,chen2017multi,xu2018pointfusion}, augmented reality \cite{marchand2015pose} and so on.  

%Object pose estimation aims to recognize the 3D location and orientation of an object in a canonical frame. It plays a significant role in numerous real-world applications, for example, robotic grasping and manipulation \cite{collet2011moped,tremblay2018deep,zhu2014single}, autonomous driving \cite{geiger2012we,chen2017multi,xu2018pointfusion} and augmented reality \cite{marchand2015pose}. An ideal solution to this problem should be robust to changes of lighting, sensor noise, occlusion scenes and truncation of objects. 

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/our_approach.png}
    \caption{
        \textbf{Pipeline of PVN3D:}  With an input RGBD image (a), we use a deep Hough voting network to predict the per-point translation offset to the selected keypoint (b). Each point on the same object votes for the selected keypoint and the center of the cluster is selected as a predicted keypoint (c). A least-squares fitting method is then applied to estimate 6D pose parameters (d)-(e). The model transformed by estimated pose parameters is shown in Figure (f). %with detected 3D keypoints in the camera coordinate system and their corresponding points in the object coordinate system (d)-(e). The model transformed by estimated pose parameters is shown in Figure (f).
    }
    \label{fig:our_approach}
\end{figure}

6DoF estimation has been proven a quite challenging problem due to variations of lighting, sensor noise, occlusion scenes and truncation of objects. Traditional methods like \cite{hinterstoisser2012model,lowe1999object} used hand-crafted features to extract the correspondence between images and object mesh models. Such empirical human-designed feature would suffer from limited performance with changing of illumination conditions and scenes with heavy occlusion. More recently, with the explosive growth of machine learning and deep learning techniques, Deep Neural Network (DNN) based methods have been introduced into this task and reveal promising improvements. \cite{wang2019densefusion,xiang2017posecnn} proposed to regress rotation and translation of objects directly with DNNs. However, these methods usually had poor generalization due to the non-linearity of the rotation space as proven in \cite{peng2019pvnet}. %in such definition, non-linearity of the rotation space makes DNN models less generalizable \cite{peng2019pvnet}.
% Technically, since there is a point transformation step involved during training, loss functions like Shape-Match-Loss  \cite{xiang2017posecnn} would make the network hard to optimize and converge.  
Instead, recent works utilized DNNs to detect 2D keypoints of an object, and computed 6D pose parameters with Perspective-n-Point (PnP) algorithms \cite{peng2019pvnet,pavlakos20176,rad2017bb8,tekin2018real}. Although these two-stage approaches performed more stable,  most of them were built on top of the 2D projection. Errors that are small in projection can be large in real 3D space. Also, different keypoints in 3D space may be overlapped after 2D projection, making them hard to be distinguished. Moreover, geometric constraint information of rigid objects would be partially lost due to projection.

% On the other hand,  with the development of inexpensive RGBD sensors, more and more RGBD datasets are available. The extra depth information enables algorithms designed for 2D to be extend to 3D space. There are already some successful solutions proposed in 3D detection like PointFusion \cite{xu2018pointfusion}, Frustum pointnets\cite{qi2018frustum} and VoteNet\cite{qi2019deep}. However, these 3D bounding box based methods can not be directly adapted for 6Dof estimation task.  The box corners are virtual points that are far away from points on the object and hard for point-based networks to aggregate scene context. The large localization error of keypoints will be propagated to the computation of 6D pose parameters. Instead, keypoints selected from vertexes on object surface will be much better. 

%On the other hand,  with the development of inexpensive RGBD sensors, more and more RGBD datasets are available. The extra depth information enables researchers to extend 2D algorithms to 3D space. For example, some successful 3D detection algorithms like PointFusion \cite{xu2018pointfusion}, Frustum pointnets\cite{qi2018frustum} and VoteNet\cite{qi2019deep} have been proposed as extension of 2D detection methods. However, the detected 3D bounding boxes are viewpoint-dependent and do not encode the precise orientation of objects. Instead, we extend 2D-keypoint-based pose estimation approach to 3D keypoint and get the precise orientation and positions of objects.

%More specifically, we develop a deep 3D keypoints Hough voting neural network to learn the point-wise 3D offset and vote for 3D keypoints, as shown in Figure \ref{fig:our_approach}.  Our key observation is a simple geometric property that positional relationship between two points of a rigid object in 3D space is fixed. Hence, given a visible point on the object surface, its coordinate and orientation can be obtained from depth images and its translation offset to selected keypoint is also fixed and learnable. Meanwhile, learning point-wise Euclidean offset is straightforward for network and easier to optimize. 

%To get the best of both worlds, we propose a 3D keypoint based method for 6Dof estimation from a single RGBD image. More specifically, we develop a deep 3D keypoints hough voting neural network to learn the point-wise 3D offset and vote for 3D keypoints. Our key observation is a simple geometric property that positional relationship between 2 points of a rigid object in 3D space is fixed. Hence, XXX. Meanwhile, the per-point Euclidean offset is straightforward for our network to learn and optimize.  To handle scenes with multi objects, we also introduced an instance semantic segmentation module into the network and jointly optimized with keypoint voting. Experimental results show that our approach outperforms current state-of-the-art methods by a remarkable margin. 

On the other hand,  with the development of inexpensive RGBD sensors, more and more RGBD datasets are available. The extra depth information allows 2D algorithms to be extend into 3D space with better performance, like PointFusion \cite{xu2018pointfusion}, Frustum pointnets\cite{qi2018frustum} and VoteNet\cite{qi2019deep}. Towards this end, we extend these 2D-keypoint-based approaches to 3D keypoint  and significantly improved the accuracy of 6DoF estimaton.  More specifically, we develop a deep 3D keypoints Hough voting neural network to learn the point-wise 3D offset and vote for 3D keypoints, as shown in Figure \ref{fig:our_approach}.  Our key observation is a simple geometric property that positional relationship between two points of a rigid object in 3D space is fixed. Hence, given a visible point on the object surface, its coordinate and orientation can be obtained from depth images and its translation offset to selected keypoint is also fixed and learnable. Meanwhile, learning point-wise Euclidean offset is straightforward for network and easier to optimize. 


To handle scenes with multiple objects, we also introduce an instance semantic segmentation module into the network and jointly optimized with keypoint voting. We find that jointly training these tasks boosts the performance of each other. Specifically, semantic information helps recognize which part a point belongs to on an object, enabling the model to better determine its translation offset to the keypoint. On the other hand, size information contains in translation offsets helps the model to distinguish objects with similar appearance but different in size, as shown in Figure \ref{fig:segmentation}.  

We further conduct experiments on YCB-Video and LineMOD datasets to evaluate our method. Experimental results show that our approach outperforms current state-of-the-art methods by a significant margin.



%To handle scenes with multiple objects, we also introduced an instance semantic segmentation module into the network and jointly optimized with keypoint voting. We find that jointly training these tasks boosts the performance of each other. Specifically, semantic information helps recognize which part a point belongs to on an object, enabling the model to better determine its translation offset to the keypoint. On the other hand, size information contains in translation offsets helps the model to distinguish objects with similar appearance but different in size. For example, the large clamp and extra-large clamp in the YCB Video dataset.
%Experimental results show that our approach outperforms current state-of-the-art methods by a significant margin.

%Hence, given the coordinate and orientation of a visible point on the object surface, obtained from depth images, the translation offset from it to the selected keypoint is also fixed and learnable.  



%Learning on point cloud also enable us to fully utilize the geometric constraint of rigid object.

%The key observation is geometric properties of rigid objects in 3D world. After recognizing a visible point of an object, we can get its coordinate and orientation. Because the positional relationship between 2 points of a rigid object is fixed, the 3D Euclidean translation offsets from such recognized points to other points on the object surface, selected as keypoints, are then determined.  Meanwhile, the per-point Euclidean offset is straightforward for our network to learn and optimize. Doing the learning on point cloud also enable us to fully utilize the geometric constraint of rigid object. Experimental results show that our approach outperforms current state-of-the-art methods by a remarkable margin. 




%with instance semantic segmentation for 6DoF pose estimation.  


%Our approach is based on some properties of rigid objects in 3D world. After recognizing a visible point of an object, we can get its coordinate and orientation. Because the positional relationship between 2 points of a rigid object is fixed, the 3D Euclidean translation offsets from such recognized points to other points on the object surface, selected as keypoints, are then determined. Under such observation, we propose a deep 3D keypoints hough voting network with instance semantic segmentation for 6DoF pose estimation. 

%The core of our proposed method is a deep hough voting neural network to learn the point-wise 3D offset and vote for 3D keytpoints. The per-point Euclidean offset is straightforward for our network to learn and optimize. Doing the learning on point cloud also enable us to fully utilize the geometric constraint of rigid object.
%Experimental results show that our approach outperforms current state-of-the-art models by a remarkable margin. 

To summarize, the main contributions of this work are as follows:
\begin{itemize}
\item A novel deep 3D keypoints Hough voting network with instance semantic segmentation for 6DoF Pose Estimation of single RGBD image .
%, which can naturally handle large occlusion scenes.
\item State-of-the-art 6DoF pose estimation performance on YCB and LINEMODE datasets.

\item An in-depth analysis of our 3D-keypoint-based method and comparison with previous approaches, demonstrating that 3D-keypoint is a key factor to boost performance for 6DoF pose estimation. We also show that jointly training 3D-keypoint and semantic segmentation can further improve the performance.
%\item An in-depth analysis of the significance of 3D-keypoint-based formulation for 6DoF Pose Estimation challenge, which shows that our 3D-keypoint-based formulation is quite better than other existing formulations.
\end{itemize}








%In the context of 3D detection in automatic driving and indoor scenes, some solutions have been proposed to detect the 8 corners of the 3D bounding box, such as 



%Therefore, directly detecting keypoints  in 3D space rather than in the projected 2D scenes is a nature improvement over previous methods and the advent of cheap RGBD sensors enables us to extend the keypoint-based method to 3D and fully utilize geometric constraint of rigid objects. 


%One direct way is to regress the rotation and translation of objects as in \cite{wang2019densefusion,xiang2017posecnn}.XXX. Other approaches \cite{peng2019pvnet,pavlakos20176,rad2017bb8,tekin2018real}utilize CNNs to detect 2D keypoints of an object, and then compute 6D pose parameters of them using Perspective-n-Point (PnP) algorithms . However XXX.  \haibin{need more work here}



%also empowers some neural-network-based method to directly regressing the rotation and translation of objects \cite{wang2019densefusion,xiang2017posecnn}. Nevertheless, non-linearity of the rotation space makes such algorithms less generalizable. Also, directly regressing to pose parameters is not straightforward for networks, because the training loss is still based on transformed points on the mesh, such as Shape-Match-Loss \cite{xiang2017posecnn}, making parameters of networks hard to optimize. 

%Instead of directly regressing pose parameters, many recent RGB-based approaches also utilize convolutional neural network (CNN) to detect 2D keypoints of an object, and then compute 6D pose parameters of them using Perspective-n-Point (PnP) algorithms \cite{peng2019pvnet,pavlakos20176,rad2017bb8,tekin2018real}. However, PnP algorithms are based on projection errors. Errors that are small in projection may be large in real 3D space. Also, different keypoints in 3D space may be overlapped after being projected to 2D, making them hard to be distinguished. What's more, geometric constraint information of rigid objects is partly lost due to projection. Therefore, detecting keypoints directly in 3D space rather than in the projected 2D scenes is quite important. The advent of cheap RGBD sensors enables us to extend the keypoint-based method to 3D so as to fully utilize geometric constraint of rigid objects. 


%In the context of 3D detection in automatic driving and indoor scenes, some solutions have been proposed to detect the 8 corners of the 3D bounding box, such as PointFusion \cite{xu2018pointfusion}, Frustum pointnets\cite{qi2018frustum} and VoteNet\cite{qi2019deep}. However, These bounding box corners are virtual points that are far away from points on the object. As a result, point-based networks are difficult to aggregate scene context in the vicinity of these virtual corner points. The large localization error of such keypoints will do harm to the compute of 6D pose parameters. Instead, keypoints selected from vertexes on object surface will be much better.



==> method_old.tex <==
\section{Method}
Given a frame of RGB-D image, the task of 6DoF pose estimation is to estimate the rigid transformation that transforms an object from its object world coordinate system to the camera world coordinate system. Such transformation $\mathbf{T} \in SE(3)$ consists of a 3D rotation $\mathbf{R} \in SO(3)$ and a translation $\mathbf{t} \in \mathbb{R}^3$.

% Figure \ref{fig:network} shows the pipeline of our proposed method. We estimate the pose of an object with a two-stage pipeline. The first stage is to propose instances with semantic labels from RGB-D images and detect 3D keypoints of each instance. The second stage is to estimate the pose of an object with a least-squares fitting method \cite{arun1987least}, given the 3D coordinate of the keypoints in the camera coordinate system and their coordinate in the object coordinate system. The innovation of our proposed method is a pioneering Deep Neural Network 3D keytpoints detection based 6D pose estimation pipeline, which, with in-depth analysis, is the best formulation among all the existing formulation for 6D pose estimation challenge.
Figure \ref{fig:network} shows the pipeline of our proposed method. We estimate the pose of an object with a two-stage pipeline. The first stage is to detect 3D keypoints of objects from a frame of RGBD image with a deep hough voting network. The second stage is to estimate the pose of an object with a least-squares fitting method \cite{arun1987least}. The innovation of our proposed method is a pioneering deep neural network 3D keypoints detection based 6D pose estimation pipeline, which, with in-depth analysis, is the best formulation among all the existing formulation for 6D pose estimation challenge.
 

\subsection{Feature Extraction Module}
The first part in Figure \ref{fig:network} shows the feature extraction module $\mathcal{F}$. Given the RGBD image in a frame of the shot, $\mathcal{F}$ first extracts the local appearance information in a RGB image and geometry information in the point cloud respectively, and then fuse them together to obtain the combined feature for each point. After the process of this module, each point $p_i$ has a feature $f_i \in \mathbb{R}^C$ of $C$ dimension.
% The first part in Figure \ref{fig:network} is a feature extraction module aiming to learn a good feature representation for each point, which will be further used to predict the semantic labels and translation offsets to the instance centers and keypoints. Given the RGB-D image in a frame of the shot, appearance feature contained in the RGB image and geometry information in the point cloud are extracted by a PSPNet\cite{zhao2017pyramid} with ResNet34\cite{resnet} and a PointNet++\cite{qi2017pointnet++} respectively, and further fused by a DenseFusion block \cite{} to obtain the combined feature for each point. After the process of this module, each point $p_i$ has a feature $f_i \in \mathbb{R}^C$ of $C$ dimension.

\subsection{3D Keypoints Detection Module}
% After obtaining the per point feature from the feature extraction backbone, we also add a header to predicted the Euclidean translation offset space from point $p_i = [x_i, f_i]$ to the target keypoints belonging to the same instance. 
With the per-point feature extracted by the feature extraction module, a 3D keypoint detection module is proposed to detect the 3D keypoints of each object. To be specific, the 3D keypoint offset module $\mathcal{G}$ predicts the per-point Euclidean translation offset from visible points to target keypoints. These visible points, together with the predicted offsets then vote for the target keypoints. The voted points are then gathered by a clustering algorithms and centers of clusters are selected as the voted keypoints.

We give a deeper view of the 3D keypoint offset module $\mathcal{G}$ as follows. Given a set of visible seed points $\{p_i\}^N_{i=1}$ and a set of selected keypoints $\{kp_j\}^M_{j=1}$ belonging to the same object instance $I$, we denote $p_i = [x_i; f_i]$ with $x_i$ the 3D coordinate and $f_i$ the extracted feature. We denote $kp_j = [y_j]$ with $y_j$ the 3D coordinate of the keypoint. The sharing keypoint voting module $\mathcal{G}$ absorbs feature $f_i$ of each seed point and generates translation offset $\{of_i^j\}_{j=1}^M$ for them, where $of_i^j$ denotes the translation offset from the $i_{th}$ seed point to the $j_{th}$ keypoint. Then the voted keypoint can be denoted as $vkp_i^{j} = x_i + of_i^{j}$. To supervise the learning of $of_i^j$, we apply a L1 loss:
\begin{equation}\label{eqn:Lofs}
    L_{\textrm{voted-keypoints}} = \frac{1}{N} \sum_{i=1}^{N} \sum_{j=1}^M ||of_i^j - of_i^{j*}|| \mathbb{I}(p_i \in I)
\end{equation}
where $of_i^{j*}$ is the ground true translation offset; $M$ is the total number of selected target keypoints; $N$ is the total number of seeds and $\mathbb{I}$ is an indicating function equates to $1$ only when point $p_i$ belongs to instance $I$, and $0$ otherwise.


\subsubsection*{\textbf{Keypoint selection}} The 3D keypoints are selected from the 3D object model. In 3D object detection algorithms \cite{qi2018frustum,xu2018pointfusion,qi2019deep}, eight corners of the 3D bounding box are selected. However, These bounding box corners are virtual points that are far away from points on the object, making point-based networks difficult to aggregate scene context in the vicinity of them. The longer distance to the object points results in larger localization errors, which may do harm to the compute of 6D pose parameters. Instead, points selected from object surface will be quite better. Therefore, we follow \cite{peng2019pvnet} and use the farthest point sampling (FPS) algorithm to select keypoints. Specifically, we initial the selection procedure by adding the center point of the object model in the empty selected keypoint set and update the selected keypoint set by adding a new point on the mesh that is farthest to all the points in the selected keypoints set repeatedly, until $M$ keypoints are obtained.


\subsection{Instance Semantic Segmentation Module}
 To handle scenes with multi objects, we also introduce an instance semantic segmentation module into the network and jointly optimized it with keypoint voting module. Given the per-point extracted feature, a semantic segmentation module $\mathcal{H}$ predict the per-point semantic labels. We supervise this module with Focal Loss \cite{lin2017focal}, denoted as $L_{\textrm{semantic}}$. Meanwhile, a center offset voting module $\mathcal{P}$ is applied to vote for centers of different object so as to distinguish different instance. Similar to the keypoint voting module $\mathcal{G}$, $\mathcal{P}$ takes in the per-point feature but predicts the Euclidean translation offset $\Delta x_i$ to the center of objects it belongs to. The learning of $\Delta x_i$ is also supervised by a L1 loss:
\begin{equation}
\label{eqn:Lctr}
    L_{\textrm{voted-center}} = \frac{1}{N} \sum_{i=1}^{N}{ ||\Delta x_i - \Delta x_i^* || \mathbb{I}(p_i \in I)
    }
\end{equation}
where $N$ denotes the total number of seed points on object surface and $\Delta x_i^*$ is the ground true translation offset from seed $p_i$ to the instance center. $\mathbb{I}$ is an indication function indicating whether point $p_i$ belongs to that instance.

During inference time, we obtain the voted center for each point with same semantic labels, then apply an easy Mean Shift \cite{cheng1995mean} clustering algorithm to split up different instances.


\renewcommand{\arraystretch}{1.5}
\begin{table*}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset.}
    \label{tab:YCB_PFM}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
        \hline
        % \multirow{2}{*}{Object}&
         \  & \multicolumn{3}{c|}{PoseCNN+ICP}&\multicolumn{3}{c|}{DenseFusion (iterative)}&\multicolumn{3}{c}{Ours}\cr\cline{1-10}
         \  &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm \cr
        \hline
        002\_master\_che\_can     &95.8 	&69.0 	&100.0 	&96.4 	&74.4 	&100.0 	&96.0 	&80.5 	&100.0 \cr%\hline
        003\_cracker\_box	        &92.7 	&80.7 	&91.6 	&95.5 	&93.9 	&99.5 	&96.1 	&94.8 	&100.0 \cr%\hline
        004\_sugar\_box	        &98.2 	&97.2 	&100.0 	&97.5 	&97.1 	&100.0 	&97.4 	&96.3 	&100.0 \cr%\hline
        005\_tomato\_soup\_can	    &94.5 	&81.6 	&96.9 	&94.6 	&88.2 	&96.9 	&95.6 	&88.6 	&98.1 \cr%\hline
        006\_mustard\_bottle	    &98.6 	&97.0 	&100.0 	&97.2 	&96.6 	&100.0 	&97.5 	&96.2 	&100.0 \cr%\hline
        007\_tuna\_fish\_can	    &97.1 	&83.1 	&100.0 	&96.6 	&82.1 	&100.0 	&95.8 	&89.0 	&100.0 \cr%\hline
        008\_pudding\_box	        &97.9 	&96.6 	&100.0 	&96.5 	&96.0 	&100.0 	&97.2 	&95.7 	&100.0 \cr%\hline
        009\_gelatin\_box	        &98.8 	&98.2 	&100.0 	&98.1 	&98.2 	&100.0 	&97.7 	&96.0 	&100.0 \cr%\hline
        010\_potted\_meat\_can	    &92.7 	&83.8 	&93.6 	&91.3 	&84.8 	&93.1 	&93.8 	&88.6 	&94.6 \cr%\hline
        011\_banana	            &97.1 	&91.6 	&99.7 	&96.6 	&78.2 	&100.0 	&96.7 	&94.0 	&100.0 \cr%\hline
        019\_pitcher\_base	    &97.8 	&96.7 	&100.0 	&97.1 	&97.3 	&100.0 	&97.4 	&96.5 	&100.0 \cr%\hline
        021\_bleach\_cleanser	    &96.9 	&92.3 	&99.4 	&95.8 	&94.9 	&100.0 	&96.0 	&93.2 	&100.0 \cr%\hline
        024\_bowl	            &81.0 	&17.5 	&54.9 	&88.2 	&5.6 	&98.8 	&90.6 	&38.6 	&85.7 \cr%\hline
        025\_mug	                &95.0 	&81.4 	&99.8 	&97.1 	&94.0 	&100.0 	&97.6 	&95.4 	&100.0 \cr%\hline
        035\_power\_drill	        &98.2 	&96.9 	&99.6 	&96.0 	&96.5 	&98.7 	&96.7 	&95.1 	&100.0 \cr%\hline
        036\_wood\_block	        &87.6 	&79.2 	&80.2 	&89.7 	&34.5 	&94.6 	&90.4 	&38.7 	&94.6 \cr%\hline
        037\_scissors	        &91.7 	&78.4 	&95.6 	&95.2 	&82.6 	&100.0 	&96.6 	&92.3 	&100.0 \cr%\hline
        040\_large\_marker	    &97.2 	&85.4 	&99.7 	&97.5 	&94.2 	&100.0 	&96.7 	&91.8 	&100.0 \cr%\hline
        051\_large\_clamp	        &75.2 	&52.6 	&74.9 	&72.9 	&31.4 	&79.2 	&93.6 	&71.6 	&98.9 \cr%\hline
        052\_extra\_large\_clamp	&64.4 	&28.7 	&48.8 	&69.8 	&30.7 	&76.3 	&85.7 	&62.7 	&90.6 \cr%\hline
        061\_foam\_brick	        &97.2 	&48.3 	&100.0 	&92.5 	&58.2 	&100.0 	&96.8 	&88.6 	&100.0 \cr\hline
        MEAN	                &93.0 	&79.3 	&93.2 	&93.0 	&76.6 	&96.8 	&{\bf95.3} 	&{\bf85.0} 	&{\bf98.2} \cr
        \hline
    \end{tabular}
\end{table*}


\subsubsection*{\textbf{Multi tasks loss}} We supervise the learning of module $\mathcal{G}$, $\mathcal{H}$ and $\mathcal{P}$ jointly with a multi-tasks loss:
\begin{equation}\label{eqn:L}
    \begin{split}
    L_{\textrm{multi-task}} = & \lambda_1 L_{\textrm{semantic}} + \lambda_2 L_{\textrm{voted-center}} \\
                     & + \lambda_3 L_{\textrm{voted-keypoints}}
    \end{split}
\end{equation}
where $\lambda_i$ is the weight for the $i_{th}$ task.

\subsection{6DoF Pose Estimation Module}
Given two point sets of an object, one from the $M$ detected keypoints $\{kp_i\}_{i=1}^{M}$ in the camera coordinate system, and another from their corresponding points $\{kp_i^{'}\}_{i=1}^{M}$ in the object coordinate system, the pose estimation module computes the pose parameters ($R$, $t$) with a least-squares fitting algorithm \cite{arun1987least}, which finds $R$ and $t$ by minimizing the following square loss:
\begin{equation} \label{eqn:lsf}
    L_{\textrm{least-squares}} = \sum_{i=1}^{M} || kp_i - (R \cdot kp^{'}_i + t) ||^2
\end{equation}
where $M$ is the number of selected keypoints of a object.

\renewcommand{\arraystretch}{1.3}
\begin{table*}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Quantitative evaluation of 6D Pose on LineMOD Dataset.}
    \label{tab:LM_PFM}
    \begin{tabular}{l|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm} }
        \hline
        % \multirow{2}{*}{Object}&
         \  & \multicolumn{3}{c|}{RGB}&\multicolumn{6}{c}{RGB-D}\cr\cline{1-10}
         \  &BB8 w ref.	&PoseCNN DeepIM	&PVNet&Implicit ICP&SSD-6D ICP &Point- Fusion	&DF(per-pixel)	&DF(iter-ative)	&Ours \cr
        \hline
        ape	            &40.4	&77.0	&43.6	&20.6	&65.0	&70.4	&79.5	&92.3	&{\bf 95.5}   \cr
        bench vise	    &91.8	&{\bf 97.5}	&99.9	&64.3	&80.0	&80.7	&84.2	&93.2	&94.5   \cr
        camera	        &55.7	&93.5	&86.9	&63.2	&78.0	&60.8	&76.5	&94.4	&94.2   \cr
        can	            &64.1	&{\bf 96.5}	&95.5	&76.1	&86.0	&61.1	&86.6	&93.1	&94.3   \cr
        cat	            &62.6	&82.1	&79.3	&72.0	&70.0	&79.1	&88.8	&96.5	&95.5   \cr
        driller	        &74.4	&95.0	&{\bf 96.4}	&41.6	&73.0	&47.3	&77.7	&87.0	&93.3   \cr
        duck	        &44.3	&77.7	&52.6	&32.4	&66.0	&63.0	&76.3	&92.3	&{\bf 94.6}   \cr
        egg box	        &57.8	&97.1	&99.2	&98.6	&{\bf 100.0}	&99.9	&99.9	&99.8	&{\bf 100.0}   \cr
        glue	        &41.2	&99.4	&95.7	&96.4	&{\bf 100.0}	&99.3	&99.4	&{\bf 100.0}	&{\bf 100.0}  \cr
        hole puncher	&67.2	&52.8	&82.0	&49.9	&49.0	&71.8	&79.0	&92.1	&{\bf 95.1}    \cr
        iron	        &84.7	&98.3	&98.9	&63.1	&78.0	&83.2	&92.1	&97.0	&92.1    \cr
        lamp	        &76.5	&97.5	&99.3	&91.7	&73.0	&62.3	&92.3	&95.3	&93.7    \cr
        phone	        &54.0	&87.7	&92.4	&71.0	&79.0	&78.8	&88.0	&92.8	&{\bf 93.6}    \cr\hline
        MEAN	        &62.7	&88.6	&86.3	&64.7	&79.0	&73.7	&86.2	&94.3	&{\bf 95.1}   \cr
        \hline  
    \end{tabular}
\end{table*}

% \renewcommand{\arraystretch}{1.5}
\newcommand{\as}{0.9}
\begin{table*}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset with diffrent formulation.}
    \label{tab:YCB_FM}
    \begin{tabular}{l|C{\as cm}|C{\as cm}|C{\as cm}|C{\as cm}|C{\as cm}|C{\as cm}|C{\as cm}}
        \hline
        % \multirow{2}{*}{Object}&
         \      & DF(RT) & DF(3D KP) &Ours(RT) &Ours(2D KP) &PVNet &Ours(Corr) &Ours(3D KP)\cr\cline{1-8}
        ADD	    &73.6	&75.9	&74.3	&77.2   &73.4	&77.0	&{\bf85.0}   \cr
        ADD-S	&91.2	&93.1	&91.8	&82.8	&-      &92.8	&{\bf95.3}   \cr
        $<$2cm	&94.8	&95.4	&95.4	&87.4	&-      &92.1	&{\bf98.2}   \cr
        \hline
    \end{tabular}
\end{table*}


%\renewcommand{\arraystretch}{1.3}
\begin{table}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Effects of different keypoint selection method.}
    \label{tab:KP_SL}
    \begin{tabular}{l|c|c|c|c }
        \hline
        \       &BBox 8 &FPS 4  &FPS 8  &FPS 12   \cr\hline
        ADD     &80.5   &82.5	&{\bf85.1}	&84.0 \cr
        ADD-S   &94.0   &94.3	&{\bf95.5}	&94.5 \cr
        $<$2cm  &95.4   &95.9	&{\bf98.2}	&96.8 \cr
        \hline  
    \end{tabular}
\end{table}


==> tmp_table_fig.tex <==
\begin{comment}
\subsection{3D Bounding Box Detection}
Recent studies in 3D object detection also detect the 8 corners of 3D bounding boxes of objects \cite{song2014sliding,song2016deep,zhou2018voxelnet,qi2018frustum}. However, the estimated 3D bounding boxes are
viewpoint-dependent and do not encode the precise orientation of objects. Most related to our methods, VoteNet \cite{qi2019deep} also proposes a deep hough voting network for 3D object detection. However, it didn't utilize the rich RGB information. It first votes for the center of objects and learned the feature of such virtual points. These virtual center further vote for the 8 corners of the bounding box. However, features of virtual center points are hard to learn and they are even farther to the corners of the bounding box, compared with points on the object. As a result, point-based networks difficult to aggregate scene context in the vicinity of these virtual corner points. Instead, we vote for 3D keypoints selected from vertexes on the object using visible points on it, which is easier for neural network to learn.
\end{comment}



%细节描述， 各个模块的网络结构， gt keypoint的生成， least square， learning时候全中选择
\renewcommand{\arraystretch}{1.5}
\newcommand{\ycbC}{0.95}
\begin{table*}[tp]
    \centering
    \fontsize{8}{8}\selectfont
    \begin{tabular}{l|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}|C{\ycbC cm}}
    \hline
                             & \multicolumn{2}{c|}{PoseCNN+ICP\cite{xiang2017posecnn}} & \multicolumn{2}{c|}{DF(iterative)\cite{wang2019densefusion}} & \multicolumn{2}{c|}{DF(iterative)\cite{wang2019densefusion}+GT} & \multicolumn{2}{c|}{PVN3D}     & \multicolumn{2}{c}{PVN3D+GT+ICP} \cr
            \hline
                             & ADD-S          & ADD(S)         & ADD-S          & ADD(S)           & ADD-S             & ADD(S)           & ADD-S         & ADD(S)        & ADD-S          & ADD(S)        \cr\hline
    002\_master\_chef\_can   & 95.8           & 68.1           & 96.4           & 73.2             & \textbf{97.1}     & 74.4             & 96.0          & 80.5          & 96.4          & \textbf{81.4} \\
    003\_cracker\_box        & 92.7           & 83.4           & 95.8           & 94.1             & 95.8              & 93.9             & \textbf{96.1} & \textbf{94.8} & 94.5          & 91.6          \\
    004\_sugar\_box          & \textbf{98.2}  & 97.1           & 97.6           & 96.5             & 98.1              & \textbf{97.6}    & 97.4          & 96.3          & 97.9          & 97.0          \\
    005\_tomato\_soup\_can   & 94.5           & 81.8           & 94.5           & 85.5             & 94.8              & 86.3             & \textbf{96.2} & 88.5          & 96.0          & \textbf{89.2} \\
    006\_mustard\_bottle     & \textbf{98.6}  & \textbf{98.0}  & 97.3           & 94.7             & 98.0              & 96.6             & 97.5          & 96.2          & 98.2          & 97.7          \\
    007\_tuna\_fish\_can     & 97.1           & 83.9           & 97.1           & 81.9             & 97.2              & 82.1             & 96.0          & 89.3          & \textbf{97.3} & \textbf{91.8} \\
    008\_pudding\_box        & 97.9           & 96.6           & 96.0           & 93.3             & 97.7              & 96.6             & 97.1          & 95.7          & \textbf{98.4} & \textbf{97.7} \\
    009\_gelatin\_box        & 98.8           & 98.1           & 98.0           & 96.7             & 98.6              & 98.3             & 97.7          & 96.1          & \textbf{98.9} & \textbf{98.5} \\
    010\_potted\_meat\_can   & 92.7           & 83.5           & 90.7           & 83.6             & 90.6              & 84.8             & 93.3          & \textbf{88.6} & \textbf{93.7} & 87.4          \\
    011\_banana              & 97.1           & 91.9           & 96.2           & 83.3             & 96.6              & 78.2             & 96.6          & 93.7          & \textbf{97.8} & \textbf{93.9} \\
    019\_pitcher\_base       & \textbf{97.8}  & 96.9           & 97.5           & 96.9             & 97.7              & \textbf{97.3}    & 97.4          & 96.5          & 97.6          & 96.8          \\
    021\_bleach\_cleanser    & 96.9           & 92.5           & 95.9           & 89.9             & 97.0              & 95.0             & 96.0          & 93.2          & \textbf{97.2} & \textbf{95.9} \\
    \textbf{024\_bowl}       & 81.0           & 81.0           & 89.5           & 89.5             & 89.7              & 89.7             & 90.2          & 90.2          & \textbf{93.3} & \textbf{93.3} \\
    025\_mug                 & 94.9           & 81.1           & 96.7           & 88.9             & 97.5              & 95.0             & 97.6          & 95.4          & \textbf{97.8} & \textbf{96.1} \\
    035\_power\_drill        & \textbf{98.2}  & \textbf{97.7}  & 96.0           & 92.7             & 97.5              & 96.5             & 96.7          & 95.1          & 97.1          & 95.6          \\
    \textbf{036\_wood\_block}& 87.6           & 87.6           & 92.8           & 92.8             & \textbf{95.6}     & \textbf{95.6}    & 90.4          & 90.4          & 92.4          & 92.4          \\
    037\_scissors            & 91.7           & 78.4           & 92.0           & 77.9             & 93.7              & 82.6             & \textbf{96.7} & \textbf{92.7} & 93.5          & 84.1          \\
    040\_large\_marker                & 97.2           & 85.3           & 97.6           & 93.0             & 97.8              & \textbf{94.2}    & 96.7          & 91.8          & \textbf{98.1} & 91.6          \\
    \textbf{051\_large\_clamp}        & 75.2           & 75.2           & 72.5           & 72.5             & 90.3              & 90.3             & 93.6          & 93.6          & \textbf{96.2} & \textbf{96.2} \\
    \textbf{052\_extra\_large\_clamp} & 64.4           & 64.4           & 69.9           & 69.9             & 74.9              & 74.9             & 88.4          & 88.4          & \textbf{93.6} & \textbf{93.6} \\
    \textbf{061\_foam\_brick}         & 97.2           & 97.2           & 92.0           & 92.0             & 92.0              & 92.0             & 96.8          & 96.8          & \textbf{98.2} & \textbf{98.2} \cr\hline
    ALL                      & 93.0           & 85.4           & 93.2           & 86.8             & 94.8              & 89.3             & 95.5          & 91.8          & \textbf{96.4} & \textbf{92.7} \cr\hline
    \end{tabular}
    \caption{Quantitative evaluation of 6D Pose (ADD-S \cite{xiang2017posecnn}, ADD(S) \cite{hinterstoisser2012model}) on YCB-Video Dataset. Objects with bold name are symmetric. +GT means inference with ground truth instance semantic segmentation.}
    \label{tab:YCB_PFM}
\end{table*}


\begin{comment}
\begin{table}[tp]
    \centering
    \fontsize{7.3}{6.5}\selectfont
    \begin{tabular}{L{1.1cm}|l|C{0.9cm}|C{0.9cm}|C{0.9cm}|C{0.9cm}}
    \hline
                                              &          & Mask R-CNN & PVN3D ($\mathbfcal{M_S}$) & PVN3D ($\mathbfcal{M_{S, K}}$) & PVN3D ($\mathbfcal{M_{S, K, C}}$) \cr\hline
    
    \multirow{2}{1.2cm}{large clamp}          & mIoU(\%) & 58.4       & 58.6             & 62.5           & \bf{70.2}                  \cr
                                              & AP(\%)   & 33.3       & 33.9             & 35.4           & \bf{46.5}                  \cr\hline
    \multirow{2}{1.2cm}{extra-large clamp}    & mIoU(\%) & 49.1       & 50.1             & 50.7           & \bf{69.0}                  \cr
                                              & AP(\%)   & 22.0       & 23.2             & 26.2           & \bf{46.6}                  \cr\hline
    \end{tabular}
    \caption{Instance semantic segmentation results of different methods on the YCB-Video Dataset. Jointly training semantic segmentation module with keypoint offset module ($\mathbfcal{M_{S,K}}$) obtains size information from the offset module and performs better, especially on large clamp and extra-large clamp. With the center voting module $\mathbfcal{M_C}$ and the Mean-Shift clustering algorithm, further improvement of performance is obtained.}
    \label{tab:SEG}
\end{table}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%\newcommand{\mnps}{0.19}
\newcommand{\mnps}{0.17}
%\newcommand{\gw}{1.27}
\newcommand{\gw}{1.17}
\begin{figure*}[htbp]
\centering
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_361.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_361.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_361.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_650.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_650.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_650.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_948.png}\\
        \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_948.png}\\
        \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_948.png}\\
        \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
    }%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_1323.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_1323.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_1323.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_2342.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_2342.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_2342.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\centering
\caption{
    \textbf{Qualitative results on the YCB-Video Dataset.} Points on different meshes are in different colors. They are projected back to the image after being transformed by the predicted pose. Images on the top row are results of DenseFusion (iterative) \cite{wang2019densefusion}. The middle row shows the results of our model without any iterative refinement procedure. The ground truths are shown in the bottom row. Our model distinguishes the challenging large clamp and extra-large clamp and estimates their poses well. Our model is also robust in heavily occluded scenes. 
}
\vspace{-0.2cm}
\label{fig:compare_fig}
\end{figure*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\mnpsCa}{0.36}
\newcommand{\gwCa}{1.1}
\begin{figure}[htbp]
\centering

\subfigure[Ground Truth]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/gt_fmsk_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%
\subfigure[PoseCNN]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/pcnn_msk_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%
\subfigure[Mask R-CNN]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/msk_cnn_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%

\subfigure[PVN3D($\mathcal{M_S}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/onlyseg_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\subfigure[PVN3D($\mathcal{M_{S,K}}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/pv_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\subfigure[PVN3D($\mathcal{M_{S,K,C}}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/cm_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\centering
\caption{
    \textbf{Qualitative results of semantic segmentation on the YCB-Video dataset.} (b) shows the ground truth label. Different objects are labeled in different color, with large clamp colored green and extra-large clamp colored orange. In (c), the simple baseline Mask-RCNN is confused by the two objects. In (d), our semantic segmentation module $\mathcal{H}$, trained separately, can not distinguish them well either. In (e), jointly training $\mathcal{H}$ with the keypoints offset voting module $\mathcal{G}$ performs better. In (f), with the voted center and Mean-Shift clustering algorithm, our model can distinguish them well.
}
\vspace{-0.2cm}
\label{fig:tmp}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
    \renewcommand{\arraystretch}{1.5}
    \begin{table*}[tp]
        \centering
        \fontsize{8.5}{8}\selectfont
        \label{tab:YCB_PFM}
        \begin{tabular}{l|c|c|c|c|c|c|c|c}
            \hline
            % \multirow{2}{*}{Object}&
             \  & \multicolumn{2}{c|}{PoseCNN+ICP\cite{xiang2017posecnn}} &\multicolumn{2}{c|}{DF(per-pixel)\cite{wang2019densefusion}} &\multicolumn{2}{c|}{DF(iterative)\cite{wang2019densefusion}}&\multicolumn{2}{c}{Ours}\cr\cline{1-9}
             \  &ADD-S &ADD &ADD-S &ADD &ADD-S &ADD &ADD-S &ADD \cr
            \hline
            002\_master\_che\_can       &95.8 	&69.0 	&95.2 	&72.0 	&{\bf 96.4} 	&74.4 	&96.0 	&{\bf 80.5}   \cr%\hline
            003\_cracker\_box	        &92.7 	&80.7 	&92.5 	&88.9 	&95.5 	&93.9 	&{\bf 96.1} 	&{\bf 94.8}   \cr%\hline
            004\_sugar\_box	            &{\bf 98.2} 	&{\bf 97.2} 	&95.1 	&93.8 	&97.5 	&97.1 	&97.4 	&96.3   \cr%\hline
            005\_tomato\_soup\_can	    &94.5 	&81.6 	&93.7 	&85.7 	&94.6 	&88.2 	&{\bf 95.6} 	&{\bf 88.6}   \cr%\hline
            006\_mustard\_bottle	    &{\bf 98.6} 	&{\bf 97.0} 	&95.9 	&93.1 	&97.2 	&96.6 	&97.5 	&96.2   \cr%\hline
            007\_tuna\_fish\_can	    &{\bf 97.1} 	&83.1 	&94.9 	&80.2 	&96.6 	&82.1 	&95.8 	&{\bf 89.0}   \cr%\hline
            008\_pudding\_box	        &{\bf 97.9} 	&{\bf 96.6} 	&94.7 	&91.1 	&96.5 	&96.0 	&97.2 	&95.7   \cr%\hline
            009\_gelatin\_box	        &{\bf 98.8} 	&{\bf 98.2} 	&95.8 	&96.3 	&98.1 	&{\bf 98.2} 	&97.7 	&96.0   \cr%\hline
            010\_potted\_meat\_can	    &92.7 	&83.8 	&90.1 	&81.9 	&91.3 	&84.8 	&{\bf 93.8} 	&{\bf 88.6}   \cr%\hline
            011\_banana	                &{\bf 97.1} 	&91.6 	&91.5 	&76.4 	&96.6 	&78.2 	&96.7 	&{\bf 94.0}   \cr%\hline
            019\_pitcher\_base	        &{\bf 97.8} 	&96.7 	&94.6 	&89.5 	&97.1 	&{\bf 97.3} 	&97.4 	&96.5   \cr%\hline
            021\_bleach\_cleanser	    &{\bf 96.9} 	&92.3 	&94.3 	&89.3 	&95.8 	&{\bf 94.9} 	&96.0 	&93.2   \cr%\hline
            \bf{024\_bowl}              &81.0 	&17.5 	&86.6 	&4.6 	&88.2 	&5.6 	&{\bf 90.6} 	&{\bf 38.6}   \cr%\hline
            025\_mug	                &95.0 	&81.4 	&95.5 	&90.6 	&97.1 	&94.0 	&{\bf 97.6} 	&{\bf 95.4}  \cr%\hline
            035\_power\_drill	        &{\bf 98.2} 	&{\bf 96.9} 	&92.4 	&92.3 	&96.0 	&96.5 	&96.7 	&95.1  \cr%\hline
            \bf{036\_wood\_block}       &87.6 	&{\bf 79.2} 	&85.5 	&34.4 	&89.7 	&34.5 	&{\bf 90.4} 	&38.7  \cr%\hline
            037\_scissors	            &91.7 	&78.4 	&96.4 	&81.8 	&95.2 	&82.6 	&{\bf 96.6} 	&{\bf 92.3}  \cr%\hline
            040\_large\_marker	        &97.2 	&85.4 	&94.7 	&91.8 	&{\bf 97.5} 	&{\bf 94.2} 	&96.7 	&91.8  \cr%\hline
            \bf{051\_large\_clamp}      &75.2 	&52.6 	&87.7 	&30.9 	&90.3 	&31.4 	&{\bf 93.6} 	&{\bf 71.6}  \cr%\hline
            \bf{052\_extra\_large\_clamp}&64.4 	&28.7 	&75.0 	&29.4 	&74.9 	&30.7 	&{\bf 85.7} 	&{\bf 62.7}  \cr%\hline
            \bf{061\_foam\_brick}       &{\bf 97.2} 	&48.3 	&92.4 	&52.3 	&92.5 	&58.2 	&96.8 	&{\bf 88.6}  \cr\hline
            ALL 	                    &93.0 	&79.3 	&92.4 	&77.1 	&94.3 	&80.2 	&{\bf 95.4} 	&{\bf 86.9}  \cr
            \hline
        \end{tabular}
        \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset. Objects with bold name are symmetric.}
    \end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% with ADD-S < 2cm
\begin{comment}
    \renewcommand{\arraystretch}{1.5}
    \begin{table*}[tp]
        \centering
        \fontsize{8.5}{8}\selectfont
        \label{tab:YCB_PFM}
        \begin{tabular}{l|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}}
            \hline
            % \multirow{2}{*}{Object}&
             \  & \multicolumn{3}{c|}{PoseCNN + ICP}&\multicolumn{3}{c|}{DenseFusion (iterative)}&\multicolumn{3}{c}{PVN3D}\cr\cline{1-10}
             \  &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm \cr
            \hline
            002\_master\_che\_can       &95.8 	&69.0 	&100.0 	&96.4 	&74.4 	&100.0 	&96.0 	&80.5 	&100.0 \cr%\hline
            003\_cracker\_box	        &92.7 	&80.7 	&91.6 	&95.5 	&93.9 	&99.5 	&96.1 	&94.8 	&100.0 \cr%\hline
            004\_sugar\_box	            &98.2 	&97.2 	&100.0 	&97.5 	&97.1 	&100.0 	&97.4 	&96.3 	&100.0 \cr%\hline
            005\_tomato\_soup\_can	    &94.5 	&81.6 	&96.9 	&94.6 	&88.2 	&96.9 	&95.6 	&88.6 	&98.1 \cr%\hline
            006\_mustard\_bottle	    &98.6 	&97.0 	&100.0 	&97.2 	&96.6 	&100.0 	&97.5 	&96.2 	&100.0 \cr%\hline
            007\_tuna\_fish\_can	    &97.1 	&83.1 	&100.0 	&96.6 	&82.1 	&100.0 	&95.8 	&89.0 	&100.0 \cr%\hline
            008\_pudding\_box	        &97.9 	&96.6 	&100.0 	&96.5 	&96.0 	&100.0 	&97.2 	&95.7 	&100.0 \cr%\hline
            009\_gelatin\_box	        &98.8 	&98.2 	&100.0 	&98.1 	&98.2 	&100.0 	&97.7 	&96.0 	&100.0 \cr%\hline
            010\_potted\_meat\_can	    &92.7 	&83.8 	&93.6 	&91.3 	&84.8 	&93.1 	&93.8 	&88.6 	&94.6 \cr%\hline
            011\_banana	                &97.1 	&91.6 	&99.7 	&96.6 	&78.2 	&100.0 	&96.7 	&94.0 	&100.0 \cr%\hline
            019\_pitcher\_base	        &97.8 	&96.7 	&100.0 	&97.1 	&97.3 	&100.0 	&97.4 	&96.5 	&100.0 \cr%\hline
            021\_bleach\_cleanser	    &96.9 	&92.3 	&99.4 	&95.8 	&94.9 	&100.0 	&96.0 	&93.2 	&100.0 \cr%\hline
            024\_bowl	                &81.0 	&17.5 	&54.9 	&88.2 	&5.6 	&98.8 	&90.6 	&38.6 	&85.7 \cr%\hline
            025\_mug	                &95.0 	&81.4 	&99.8 	&97.1 	&94.0 	&100.0 	&97.6 	&95.4 	&100.0 \cr%\hline
            035\_power\_drill	        &98.2 	&96.9 	&99.6 	&96.0 	&96.5 	&98.7 	&96.7 	&95.1 	&100.0 \cr%\hline
            036\_wood\_block	        &87.6 	&79.2 	&80.2 	&89.7 	&34.5 	&94.6 	&90.4 	&38.7 	&94.6 \cr%\hline
            037\_scissors	            &91.7 	&78.4 	&95.6 	&95.2 	&82.6 	&100.0 	&96.6 	&92.3 	&100.0 \cr%\hline
            040\_large\_marker	        &97.2 	&85.4 	&99.7 	&97.5 	&94.2 	&100.0 	&96.7 	&91.8 	&100.0 \cr%\hline
            051\_large\_clamp	        &75.2 	&52.6 	&74.9 	&90.3 	&31.4 	&98.0  	&93.6 	&71.6 	&98.9 \cr%\hline
            052\_extra\_large\_clamp	&64.4 	&28.7 	&48.8 	&74.9 	&30.7 	&86.4  	&85.7 	&62.7 	&90.6 \cr%\hline
            061\_foam\_brick	        &97.2 	&48.3 	&100.0 	&92.5 	&58.2 	&100.0 	&96.8 	&88.6 	&100.0 \cr\hline
            MEAN	                    &93.0 	&79.3 	&93.2 	&94.0 	&76.6 	&98.4  	&{\bf95.3} 	&{\bf85.0} 	&{\bf98.2} \cr
            \hline
        \end{tabular}
        \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset. Objects with bold name are symmetric.}
    \end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%

\renewcommand{\arraystretch}{1.5}
\begin{table*}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset with diffrent formulation.}
    \label{tab:YCB_FM}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        % \multirow{2}{*}{Object}&
         \  & \multicolumn{2}{c|}{DF(RT)} & \multicolumn{2}{c|}{DF(3D KP)} 
         &\multicolumn{2}{c|}{Ours(RT)}&\multicolumn{2}{c|}{Ours(2D KP)}
         &\multicolumn{2}{c|}{Ours(Corr)}&\multicolumn{2}{c}{Ours(3D KP)}\cr\cline{1-13}
         \  &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD\cr
        \hline
        002\_master\_che\_can     &95.8 	&69.0 	&100.0 	&96.4 	&74.4 	&100.0 	&96.0 	&80.5 	&100.0 \cr%\hline
        003\_cracker\_box	        &92.7 	&80.7 	&91.6 	&95.5 	&93.9 	&99.5 	&96.1 	&94.8 	&100.0 \cr%\hline
        004\_sugar\_box	        &98.2 	&97.2 	&100.0 	&97.5 	&97.1 	&100.0 	&97.4 	&96.3 	&100.0 \cr%\hline
        005\_tomato\_soup\_can	    &94.5 	&81.6 	&96.9 	&94.6 	&88.2 	&96.9 	&95.6 	&88.6 	&98.1 \cr%\hline
        006\_mustard\_bottle	    &98.6 	&97.0 	&100.0 	&97.2 	&96.6 	&100.0 	&97.5 	&96.2 	&100.0 \cr%\hline
        007\_tuna\_fish\_can	    &97.1 	&83.1 	&100.0 	&96.6 	&82.1 	&100.0 	&95.8 	&89.0 	&100.0 \cr%\hline
        008\_pudding\_box	        &97.9 	&96.6 	&100.0 	&96.5 	&96.0 	&100.0 	&97.2 	&95.7 	&100.0 \cr%\hline
        009\_gelatin\_box	        &98.8 	&98.2 	&100.0 	&98.1 	&98.2 	&100.0 	&97.7 	&96.0 	&100.0 \cr%\hline
        010\_potted\_meat\_can	    &92.7 	&83.8 	&93.6 	&91.3 	&84.8 	&93.1 	&93.8 	&88.6 	&94.6 \cr%\hline
        011\_banana	            &97.1 	&91.6 	&99.7 	&96.6 	&78.2 	&100.0 	&96.7 	&94.0 	&100.0 \cr%\hline
        019\_pitcher\_base	    &97.8 	&96.7 	&100.0 	&97.1 	&97.3 	&100.0 	&97.4 	&96.5 	&100.0 \cr%\hline
        021\_bleach\_cleanser	    &96.9 	&92.3 	&99.4 	&95.8 	&94.9 	&100.0 	&96.0 	&93.2 	&100.0 \cr%\hline
        024\_bowl	            &81.0 	&17.5 	&54.9 	&88.2 	&5.6 	&98.8 	&90.6 	&38.6 	&85.7 \cr%\hline
        025\_mug	                &95.0 	&81.4 	&99.8 	&97.1 	&94.0 	&100.0 	&97.6 	&95.4 	&100.0 \cr%\hline
        035\_power\_drill	        &98.2 	&96.9 	&99.6 	&96.0 	&96.5 	&98.7 	&96.7 	&95.1 	&100.0 \cr%\hline
        036\_wood\_block	        &87.6 	&79.2 	&80.2 	&89.7 	&34.5 	&94.6 	&90.4 	&38.7 	&94.6 \cr%\hline
        037\_scissors	        &91.7 	&78.4 	&95.6 	&95.2 	&82.6 	&100.0 	&96.6 	&92.3 	&100.0 \cr%\hline
        040\_large\_marker	    &97.2 	&85.4 	&99.7 	&97.5 	&94.2 	&100.0 	&96.7 	&91.8 	&100.0 \cr%\hline
        051\_large\_clamp	        &75.2 	&52.6 	&74.9 	&72.9 	&31.4 	&79.2 	&93.6 	&71.6 	&98.9 \cr%\hline
        052\_extra\_large\_clamp	&64.4 	&28.7 	&48.8 	&69.8 	&30.7 	&76.3 	&85.7 	&62.7 	&90.6 \cr%\hline
        061\_foam\_brick	        &97.2 	&48.3 	&100.0 	&92.5 	&58.2 	&100.0 	&96.8 	&88.6 	&100.0 \cr\hline
        MEAN	                &93.0 	&79.3 	&93.2 	&93.0 	&76.6 	&96.8 	&{\bf95.3} 	&{\bf85.0} 	&{\bf98.2} \cr
        \hline
    \end{tabular}
\end{table*}
%%%%

